Understanding the Behaviors of BERT in Ranking

This paper studies the performances and behaviors of BERT in ranking tasks. We explore several different ways to leverage the pre-trained BERT and fine-tune it on two ranking tasks: MS MARCO passage reranking and TREC Web Track ad hoc document ranking. Experimental results on MS MARCO demonstrate the strong effectiveness of BERT in question-answering focused passage ranking tasks, as well as the fact that BERT is a strong interaction-based seq2seq matching model. Experimental results on TREC show the gaps between the BERT pre-trained on surrounding contexts and the needs of ad hoc document ranking. Analyses illustrate how BERT allocates its attentions between query-document tokens in its Transformer layers, how it prefers semantic matches between paraphrase tokens, and how that differs with the soft match patterns learned by a click-trained neural ranker.

==> archive/eva.tex <==

\subsection{Learned Term Matches}

In all 6980 queries on the \textbf{Eval} set, there are 1539 queries both Conv-KNRM and BERT(Last-Int) perform better than LeToR and there are 401 queries they both failed. The top-2 win/loss queries and their relevant documents are as follows:

% \input{case/case_win_0.tex}

% \space

% \input{case/case_win_1.tex}

% \space

% \input{case/case_lose_0.tex}

% \space

% \input{case/case_loss_1.tex}

% \space
    
    
    
    
        

% \cx{Show cases of top contributing words or n-grams in Conv-KNRM and MS MARCO}
% \cx{Show the overlap of winning queries in Conv-KNRM and MS MARCO (winning queries are those they perform better than LeToR. and also overlap of losing queries from the two methods.}
% \cx{Show the overlap of those queries' top contributing terms (document terms that lead to the highest ranking score improvents (original doc ranking score - doc ranking score with the term/ngram removed.}


% \begin{figure}
%     \centering
%     \includegraphics[width=120]{figure/var_remove_word.png}
%     \caption{Variance by removing one word from doc}
%     \label{fig:my_label}
% \end{figure}





% Query: solar panel

% Document: what is a solar panel?what is a solar panel? a solar panel is a device that collects photons of sunlight

% The heatmap of term level relevance of Conv-knrm shows that such pairs have low level of similarities.



==> case/case_lose_0.tex <==
    Q: what is a macchiato coffee drink
    
    D: 1. Latte, in Italian, means milk while Macchiato means marked or spotted. 2. Latte is basically coffee and milk, Macchiato is coffee with milk but the milk is added as a visible mark. 3. Latte, essentially refers to the ingredient of the drink while macchiato refers to the appearance of the drink.

    Conv-KNRM top matches: 
        (a macchiato coffee, macchiato)
        (macchiato coffee drink, visible)
        (what is, macchiato is)
        (a macchiato coffee, macchiato)
        (is a, macchiato is)
        
    Bert Key Words: (original 0.9737)
      
        macchiato: 3.7284e-05
      
        coffee: 0.1378
      
        drink: 0.9243
    
    Bert on Removing: (original 0.9737)
      
        macchiato: 3.7284e-05
      
        visible: 0.9815
        

==> case/case_loss_1.tex <==
    Q: does estrogen make me start my period
    
    D: 1 I was given estrogen to stop my period, but its giving me headaches. Dr. Michael Kleerekoper Dr. Kleerekoper. 1 doctor agreed: Period: Please report this to your gynecologist and follow her/his advice.

    Conv-KNRM top matches: 
        (make me, estrogen to)
        (me start, report)
        (estrogen make, advice)
        (make me, agreed period)

        
    Bert Key Words: (original 0.9982)
   
        estrogen to: 4.1099e-04
    
    Bert on Removing: (original 0.9982)
    
        estrogen to: 4.1099e-04
    
        report: 0.9885
    
        advice: 0.9924
    
        period: 0.9812

==> case/case_win_0.tex <==
    Q: who sings arabian nights aladdin
    
    D: 01:34. Arabian Nights is the opening song from Aladdin, with music by Alan Menken and lyrics by Howard Ashman. It was performed by The Peddler (singing voice by the late Bruce Adler). Howard Ashman and Alan Menken had written several reprises, but they were ultimately cut from the final film.

    Conv-KNRM top matches: 
        (who sings, peddler singing)
        (sings arabian, menken had)
        (nights aladdin, singing)
        (arabian nights, performed by)
        (sings arabian, performed by)
        (sings arabian, final film)
        
    Bert Key Words: (original 0.9982)
    
        arabian nights: 0.0094
    
    Bert on Removing: (original 0.9982)
    
        peddler singing: 0.9977
        
        menken and: 0.9985
        
        singing: 0.9984
        
        performed by: 0.9981
        
        final film: 0.9982

==> case/case_win_1.tex <==
    Q: meaning of prima donna
    
    D: Define prima donna. prima donna synonyms, prima donna pronunciation, prima donna translation, English dictionary definition of prima donna. n. 1. The leading woman soloist in an opera company. 2. A temperamental, conceited person. n , pl prima donnas 1. a female operatic star; diva 2.

    Conv-KNRM top matches: 
        (of prima, donna prima)
        (of prima, diva 2)
        (meaning of prima, donnas)
        
    Bert Key Words: (original 0.9982)
    
        prima: 0.9861
        
        prima donna: 0.5840
    
    Bert on Removing: (original 0.9982)
    
        donna prima: 0.9986
        
        diva 2: 0.9985
        
        donnas: 0.9971

==> table/clueweb.tex <==
\begin{table*}[h]
    \centering
    
\caption{Ranking Performances on ClueWeb09-B. Relative performances are compared against feature-based learning to rank (\texttt{LeToR}). All neural methods are pre-trained on MS MARCO passage ranking labels except \texttt{Conv-KNRM (Bing)}.
\cx{Show only NDCG and ERR @20. without W/T/L. Discard the validation split performance. We are focusing on MARCO and the analyses. Merge the rest of this table to Table 1.}
    \label{tab:clueweb}}

\begin{tabular}{l|cc|cc|c||cc|cc|c}
\hline \hline
 & \multicolumn{5}{c|}{\textbf{Validation Splits}} & \multicolumn{5}{|c}{\textbf{Evaluation Splits}} \\ \hline
\bf{Method}& \multicolumn{2}{c}{\bf{NDCG@ 1}}& \multicolumn{2}{c}{\bf{NDCG@20}}&\bf{W/T/L}&\multicolumn{2}{c}{\bf{NDCG@ 1}}& \multicolumn{2}{c}{\bf{NDCG@20}}&\bf{W/T/L}\\ \hline

\texttt{Base} \\
\texttt{LeToR} \\ \hline
\texttt{K-NRM} \\

\texttt{Conv-KNRM (MARCO)}
 & ${0.2100}^{\dagger \ddagger }$ & $ +7.92\%  $
 
 
 & $0.2167$ & --  & $0.2118$ & --  & --/--/-- \\
\texttt{Conv-KNRM (Bing)}
\\ \hline

\texttt{BERT (Rep)}
 & ${0.1806}$ & $ -25.69\%  $ 

 & ${0.1725}$ & $ -22.78\%  $ 

& 58/33/106

 & ${0.1369}$ & $ -36.83\%  $ 

 & ${0.1479}$ & $ -30.16\%  $ 

& 49/32/116

\\ \hline
\texttt{BERT (Feature)} 
 & ${0.1920}$ & $ -20.99\%  $

 & ${0.1948}$ & $ -12.80\%  $

& 76/33/88

 & ${0.1972}$ & $ -9.01\%  $

 & ${0.1937}$ & $-8.56\%  $

& 78/31/88 \\

\texttt{BERT (Last-Int)}
 & ${0.2835}$ & $ +16.67\%  $ 

 & ${0.2673}^{\dagger }$ & $ +19.69\%  $ 

& 113/31/53

 & ${0.2603}$ & $ +7.12\%  $ 

 & ${0.2407}^{\dagger }$ & $ +7.76\%  $ 

& 94/32/71

\\

\texttt{BERT (Mult-Int)}
 & ${0.2957}$ & $ +21.71\%  $ 

 & ${0.2607}$ & $ +16.72\%  $ 

& 85/10/82

 & ${0.2541}$ & $ +17.27\%  $ 

 & ${0.2407}^{\dagger }$ & $ +13.60\%  $ 

& 101/30/66

\\
\texttt{BERT (Term-Trans)}
 & ${0.3170}^{\dagger }$ & $ +30.46\%  $ 

 & ${0.2670}^{\dagger }$ & $ +19.54\%  $ 

& 111/29/57

 & ${0.2315}$ & $ +6.80\%  $ 

 & ${0.2339}$ & $ +10.41\%  $ 

& 103/27/67
\\

\hline \hline

\end{tabular}
\end{table*}

==> table/remove_word.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance of \texttt{BERT (Last-Int)} on sampled MARCO validation queries with stop words or marker tokens removed from candidate passages. Relative percentages show the lost accuracy from word removal.
    \label{tab:wordremove}
    }
    \begin{tabular}{l|c|c}
        \hline \hline
        \textbf{Method} & \multicolumn{2}{|c}{\textbf{MRR@10 (Dev)}} \\ \hline
        Original Document & 0.3577 &  \\ \hline
        Remove Stopwords & 0.3512  & \\
        Remove Markers & 0.3092  & \\ 
        \hline \hline 
    \end{tabular}
\end{table}
